Abstract Continuation Semantics for Multiparty Interactions in Process Calculi based on CCS

We develop denotational and operational semantics designed with continuations for process calculi based on CCS extended with mechanisms offering support for multiparty interactions. We investigate the abstractness of this continuation semantics. We show that our continuation-based denotational models are weakly abstract with respect to the corresponding operational models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{M. Marin, L. Leu\c{s}tean (Eds.):\\ 
8th Symposium on Working Formal Methods (FROM 2024)\\
EPTCS 410, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.410.2}{10.4204/EPTCS.410.2}}
\pdfoutput=1

